American Sign Language fingerspelling recognition from video: Methods for unrestricted recognition and signer-independence

In this thesis, we study the problem of recognizing video sequences of fingerspelled letters in American Sign Language (ASL). Fingerspelling comprises a significant but relatively understudied part of ASL, and recognizing it is challenging for a number of reasons: It involves quick, small motions that are often highly coarticulated; it exhibits significant variation between signers; and there has been a dearth of continuous fingerspelling data collected. In this work, we propose several types of recognition approaches, and explore the signer variation problem. Our best-performing models are segmental (semi-Markov) conditional random fields using deep neural network-based features. In the signer-dependent setting, our recognizers achieve up to about 8% letter error rates. The signer-independent setting is much more challenging, but with neural network adaptation we achieve up to 17% letter error rates.

==> app_scrf.tex <==
\chapter{A semi-Markov CRF approach}
\label{sec:app_scrf}

We begin by defining the problem and our notation.  Let the sequence of visual observations for a given video (corresponding to a single word) be $O = o_1, \ldots, o_T$, where each $o_t$ is a multidimensional image descriptor for frame $t$.  Our goal is to predict the label (letter) sequence.  Ideally we would like to predict the best label sequence, marginalizing out different possible label start and end times, but in practice we use the typical approach of predicting the best sequence of frame labels $S = s_1, \ldots, s_T$.  We predict $S$ by maximizing its conditional probability under our model, $\hat{S} = \text{argmax}_S P(S|O)$.
In generative models like HMMs, we have a joint model $P(S,O)$ and we make a prediction using Bayes' rule.
In conditional models we directly represent the conditional distribution $P(S|O)$.  For example, in a typical linear-chain CRF, we have:
\[
p(S|O) = \frac{1}{Z(O)}\exp\left(\sum_{v,k}\lambda_k f_k(S_v,O_v) + \sum_{e,k}\mu_k g_k(S_e)\right)
\]
where $Z(O)$ is the partition function, $f_k$ are the ``node'' feature
functions that typically correspond to the state in a single frame
$S_v$ and its corresponding observation $O_v$, $g_k$ are ``edge''
feature functions corresponding to inter-state edges, $e$
  ranges over pairs of frames and $S_e$ is the pair of states
  corresponding to $e$, and $\lambda_k$ and $\mu_k$ are the 
%corresponding 
weights.  
%In a linear-chain CRF, the conditional distribution factorizes over individual frames; that is, $v$ ranges over the frames and $e$ over the sequence of frame pairs.

It may be more natural to consider feature functions that span entire
segments corresponding to the same label.  Semi-Markov
CRFs~\cite{sarawagisemi}, also referred to as segmental
CRFs~\cite{zweig} or SCRFs, provide this ability.  
%Figure~\ref{f:SCRF} shows a SCRF for fingerspelled letter recognition, with an example labeling and segmentation.

%\begin{figure}[t]
%\centering
%\includegraphics[width=0.45\textwidth]{figs/SCRF2_small.pdf}
%\caption{SCRF for fingerspelled letter recognition, with an example fingerspelled letter sequence '-V-I-T-A-'.  Dotted lines show one possible segmentation.  Feature functions are defined over edges between labels and over segments of tobservations.}
%\label{f:SCRF}
%\end{figure}

Figure~\ref{fig:s-crf} illustrates the SCRF notation, which we now describe.
In a SCRF, we consider the segmentation to be a latent variable and sum over all possible segmentations of the observations corresponding to a given label sequence to get the conditional probability of the label sequence $S = s_1, \ldots, s_L$, where the length of $S$ is now the (unknown) number of distinct labels $L$:
\[
p(S|O) = \frac{\sum_{q ~\text{s.t.}~ |q|=|S|} \exp\left(\sum_{e \in q,k} \lambda_k f_k (s_l^e,s_r^e,O_e)\right)}{\sum_{S^\prime} \sum_{q~\text{s.t.} |q|=|S^\prime|} \exp\left(\sum_{e \in q,k} \lambda_k f_k (s_l^e,s_r^e,O_e)\right)}
\]
Here, $S'$ ranges over all possible state (label) sequences, $q$ is a segmentation of the observation sequence whose length (number of segments) must be the same as the number of states in $S$ (or $S^\prime$), $e$ ranges over all state pairs in $S$, $s_l^e$ is the state which is on the left of an edge, $s_r^e$ is the state on the right of an edge, and $O_e$ is the multi-frame observation segment associated with $s_r^e$.
%the state on the right of the edge $e$.  
In our work, we use a baseline frame-based recognizer to generate a set of candidate segmentations of $O$, and sum only over those candidate segmentations.  In principle the inference over all possible segmentations can be done, but typically this is only feasible for much smaller search spaces than ours. 

\begin{comment}\subsection{Letter model and transition model}
In the formulation above, each state could represent either letter or transition of two letter pairs. For each case, we need to define different feature functions.
\subsection{Feature functions for letter model}
\end{comment}



\begin{figure*}
%  \begin{minipage}[c]{.27\linewidth}
%    \includegraphics[width=0.99\textwidth]{figs/asl-alphabet-wiki}
%  \end{minipage}\hspace{2em}%
%  \begin{minipage}[c]{.68\linewidth}
  \centering
  \begin{tikzpicture}[scale=.6]
    % frames
    \foreach \t in {1,2,3,6,7,8,9,12,13}{
      \draw[fill=gray] (\t,0) rectangle ++(.8,-3);
      \node at (5,-1.5) {\large \ldots};
      \node at (11,-1.5) {\large \ldots};
      \node at (15,-1.5) {\large \ldots};
    }
    % observations
    \node at (1.4,-3.4) {$o_1$};
    \node at (2.4,-3.4) {$o_2$};
    \node at (3.4,-3.4) {$o_3$};
    \node[text width=7em] (labelvis) at (-1,-2) {visual\\feature\\vectors};
    \coordinate (s1) at (1,1.5);
    \coordinate (e1) at (7.8,1.5);
    \coordinate (s2) at (8,1.5);
    \coordinate (e2) at (12.8,1.5);
    \coordinate (s3) at (13,1.5);
    % segments
    \draw[thick,rounded corners] ($(s1) - (0,.5)$) -- ++(0,.5) --
    (e1)
    node[midway,circle,fill=black,inner sep=2pt,name=seg1] {}  -- ++(0,-.5);
    \draw[thick,rounded corners] ($(s2) - (0,.5)$) -- ++(0,.5) -- (e2)
    node[midway,circle,fill=black,inner sep=2pt,name=seg2] {} -- ++(0,-.5);
    \draw[thick,rounded corners] ($(s3) - (0,.5)$) -- ++(0,.5) -- ++(2,0)
    node[midway,circle,fill=black,inner sep=2pt,name=seg3] {};
    % observation sequences
    \draw[decorate,decoration={brace,amplitude=5pt}] ($(e1) - (0,5)$)
    -- ($(s1) - (0,5)$) node [midway,below=4pt] {$O_{(1)}$};
    \draw[decorate,decoration={brace,amplitude=5pt}] ($(e2) - (0,5)$)
    -- ($(s2) - (0,5)$) node [midway,below=4pt] {$O_{(2)}$};
    % states
    \node[draw] (state1) at ($(seg1) + (0,2)$) {$s_1$};
    \node[draw] (state0) at ($(state1) - (4,0)$) {$s_0$};
    \node[draw] (state2) at ($(seg2) + (0,2)$) {$s_2$};
    \node[draw] (state3) at ($(seg3) + (0,2)$) {$s_3$};
    \path let \p1=(labelvis), \p2=(state0) in node[text width=7em]  at(\x1,\y2)
 {state\\labels};
    \draw (state1) -- (seg1);
    \draw (state2) -- (seg2);
    \draw (state3) -- (seg3);
    \path let \p1=(labelvis), \p2=(s1) in node[text width=7em]
    at(\x1,\y2)  {segmentation $q$};
    % edges
    \draw (state0) -- (state1) node[midway,below] {$e_1$};
    \draw (state1)--(state2) node[midway,below] {$e_2$};
    \draw (state2)--(state3) node[midway,below] {$e_3$};
    \draw (state3) -- ++(1.5,0);
    % states per edge
    \path (state0) -- ++(0,1) node {$s_l^{(1)}$};
    \path (state1) -- ++(0,1) node {$s_r^{(1)}=s_l^{(2)}$};
    \path (state2) -- ++(0,1) node {$s_r^{(2)}=s_l^{(3)}$};
    % times
    {\tiny
    \node at (1.5,.5) {$t(1)$};
    \node at (7.5,.5) {$T(1)$};
    \node at (8.5,.5) {$t(2)$};
    \node at (12.5,.5) {$T(2)$};
    \node at (13.5,.5) {$t(3)$};
  }
  \end{tikzpicture}
 % \end{minipage}

%  \begin{minipage}[t]{.27\linewidth}
%    \caption{The ASL fingerspelled alphabet. All of the
%  letters except for J and Z are static. [From Wikipedia]}
%\label{f:alphabet}
%  \end{minipage}\hspace{2em}%
%  \begin{minipage}[t]{.68\linewidth}
    \caption[Illustration of SCRF notation]{Illustration of SCRF notation. For example, edge $e_2$ is
associated with the ``left state'' $s_l^{(2)}$, the ``right state'' $s_r^{(2)}$, and the 
    segment of observations $O_{(2)}$ spanning frames $t(2)$ through
    $T(2)$. 
%\karencomment{[Changed notation for O in fig. to match
%equations. --KL]}
}
%; the observation     sequence for this segment is $O_b=(o_{t(2)},\ldots,o_{T(2)})$.}
% The   segment corresponds to state $s_r^{(2)}=s_2$, following state $s_l^{(2)}=s_1$.}
  \label{fig:s-crf}
%  \end{minipage}
\end{figure*}




==> chap1.tex <==
%% This is an example first chapter.  You should put chapter/appendix that you
%% write into a separate file, and add a line \include{yourfilename} to
%% main.tex, where `yourfilename.tex' is the name of the chapter/appendix file.
%% You can process specific files by typing their names in at the 
%% \files=
%% prompt when you run the file main.tex through LaTeX.
\chapter{Introduction}

Micro-optimization is a technique to reduce the overall operation count of
floating point operations.  In a standard floating point unit, floating
point operations are fairly high level, such as ``multiply'' and ``add'';
in a micro floating point unit ($\mu$FPU), these have been broken down into
their constituent low-level floating point operations on the mantissas and
exponents of the floating point numbers.

Chapter two describes the architecture of the $\mu$FPU unit, and the
motivations for the design decisions made.

Chapter three describes the design of the compiler, as well as how the
optimizations discussed in section~\ref{ch1:opts} were implemented.

Chapter four describes the purpose of test code that was compiled, and which
statistics were gathered by running it through the simulator.  The purpose
is to measure what effect the micro-optimizations had, compared to
unoptimized code.  Possible future expansions to the project are also
discussed.

\section{Motivations for micro-optimization}

The idea of micro-optimization is motivated by the recent trends in computer
architecture towards low-level parallelism and small, pipelineable
instruction sets \cite{patterson:risc,rad83}.  By getting rid of more
complex instructions and concentrating on optimizing frequently used
instructions, substantial increases in performance were realized.

Another important motivation was the trend towards placing more of the
burden of performance on the compiler.  Many of the new architectures depend
on an intelligent, optimizing compiler in order to realize anywhere near
their peak performance
\cite{ellis:bulldog,pet87,coutant:precision-compilers}.  In these cases, the
compiler not only is responsible for faithfully generating native code to
match the source language, but also must be aware of instruction latencies,
delayed branches, pipeline stages, and a multitude of other factors in order
to generate fast code \cite{gib86}.

Taking these ideas one step further, it seems that the floating point
operations that are normally single, large instructions can be further broken
down into smaller, simpler, faster instructions, with more control in the
compiler and less in the hardware.  This is the idea behind a
micro-optimizing FPU; break the floating point instructions down into their
basic components and use a small, fast implementation, with a large part of
the burden of hardware allocation and optimization shifted towards
compile-time.

Along with the hardware speedups possible by using a $\mu$FPU, there are
also optimizations that the compiler can perform on the code that is
generated.  In a normal sequence of floating point operations, there are
many hidden redundancies that can be eliminated by allowing the compiler to
control the floating point operations down to their lowest level.  These
optimizations are described in detail in section~\ref{ch1:opts}.

\section{Description of micro-optimization}\label{ch1:opts}

In order to perform a sequence of floating point operations, a normal FPU
performs many redundant internal shifts and normalizations in the process of
performing a sequence of operations.  However, if a compiler can
decompose the floating point operations it needs down to the lowest level,
it then can optimize away many of these redundant operations.  

If there is some additional hardware support specifically for
micro-optimization, there are additional optimizations that can be
performed.  This hardware support entails extra ``guard bits'' on the
standard floating point formats, to allow several unnormalized operations to
be performed in a row without the loss information\footnote{A description of
the floating point format used is shown in figures~\ref{exponent-format}
and~\ref{mantissa-format}.}.  A discussion of the mathematics behind
unnormalized arithmetic is in appendix~\ref{unnorm-math}.

The optimizations that the compiler can perform fall into several categories:

\subsection{Post Multiply Normalization}

When more than two multiplications are performed in a row, the intermediate
normalization of the results between multiplications can be eliminated.
This is because with each multiplication, the mantissa can become
denormalized by at most one bit.  If there are guard bits on the mantissas
to prevent bits from ``falling off'' the end during multiplications, the
normalization can be postponed until after a sequence of several
multiplies\footnote{Using unnormalized numbers for math is not a new idea; a
good example of it is the Control Data CDC 6600, designed by Seymour Cray.
\cite{thornton:cdc6600} The CDC 6600 had all of its instructions performing
unnormalized arithmetic, with a separate {\tt NORMALIZE} instruction.}.

% This is an example of how you would use tgrind to include an example
% of source code; it is commented out in this template since the code
% example file does not exist.  To use it, you need to remove the '%' on the
% beginning of the line, and insert your own information in the call.
%
%\tagrind[htbp]{code/pmn.s.tex}{Post Multiply Normalization}{opt:pmn}

As you can see, the intermediate results can be multiplied together, with no
need for intermediate normalizations due to the guard bit.  It is only at
the end of the operation that the normalization must be performed, in order
to get it into a format suitable for storing in memory\footnote{Note that
for purposed of clarity, the pipeline delays were considered to be 0, and
the branches were not delayed.}.

\subsection{Block Exponent}

In a unoptimized sequence of additions, the sequence of operations is as
follows for each pair of numbers ($m_1$,$e_1$) and ($m_2$,$e_2$).
\begin{enumerate}
  \item Compare $e_1$ and $e_2$.
  \item Shift the mantissa associated with the smaller exponent $|e_1-e_2|$
        places to the right.
  \item Add $m_1$ and $m_2$.
  \item Find the first one in the resulting mantissa.
  \item Shift the resulting mantissa so that normalized
  \item Adjust the exponent accordingly.
\end{enumerate}

Out of 6 steps, only one is the actual addition, and the rest are involved
in aligning the mantissas prior to the add, and then normalizing the result
afterward.  In the block exponent optimization, the largest mantissa is
found to start with, and all the mantissa's shifted before any additions
take place.  Once the mantissas have been shifted, the additions can take
place one after another\footnote{This requires that for n consecutive
additions, there are $\log_{2}n$ high guard bits to prevent overflow.  In
the $\mu$FPU, there are 3 guard bits, making up to 8 consecutive additions
possible.}.  An example of the Block Exponent optimization on the expression
X = A + B + C is given in figure~\ref{opt:be}.

% This is an example of how you would use tgrind to include an example
% of source code; it is commented out in this template since the code
% example file does not exist.  To use it, you need to remove the '%' on the
% beginning of the line, and insert your own information in the call.
%
%\tgrind[htbp]{code/be.s.tex}{Block Exponent}{opt:be}

\section{Integer optimizations}

As well as the floating point optimizations described above, there are
also integer optimizations that can be used in the $\mu$FPU.  In concert
with the floating point optimizations, these can provide a significant
speedup.  

\subsection{Conversion to fixed point}

Integer operations are much faster than floating point operations; if it is
possible to replace floating point operations with fixed point operations,
this would provide a significant increase in speed.

This conversion can either take place automatically or or based on a
specific request from the programmer.  To do this automatically, the
compiler must either be very smart, or play fast and loose with the accuracy
and precision of the programmer's variables.  To be ``smart'', the computer
must track the ranges of all the floating point variables through the
program, and then see if there are any potential candidates for conversion
to floating point.  This technique is discussed further in
section~\ref{range-tracking}, where it was implemented.

The other way to do this is to rely on specific hints from the programmer
that a certain value will only assume a specific range, and that only a
specific precision is desired.  This is somewhat more taxing on the
programmer, in that he has to know the ranges that his values will take at
declaration time (something normally abstracted away), but it does provide
the opportunity for fine-tuning already working code.

Potential applications of this would be simulation programs, where the
variable represents some physical quantity; the constraints of the physical
system may provide bounds on the range the variable can take.
\subsection{Small Constant Multiplications}

One other class of optimizations that can be done is to replace
multiplications by small integer constants into some combination of
additions and shifts.  Addition and shifting can be significantly faster
than multiplication.  This is done by using some combination of
\begin{eqnarray*}
a_i & = & a_j + a_k \\
a_i & = & 2a_j + a_k \\
a_i & = & 4a_j + a_k \\
a_i & = & 8a_j + a_k \\
a_i & = & a_j - a_k \\
a_i & = & a_j \ll m \mbox{shift}
\end{eqnarray*}
instead of the multiplication.  For example, to multiply $s$ by 10 and store
the result in $r$, you could use:
\begin{eqnarray*}
r & = & 4s + s\\
r & = & r + r
\end{eqnarray*}
Or by 59:
\begin{eqnarray*}
t & = & 2s + s \\
r & = & 2t + s \\
r & = & 8r + t
\end{eqnarray*}
Similar combinations can be found for almost all of the smaller
integers\footnote{This optimization is only an ``optimization'', of course,
when the amount of time spent on the shifts and adds is less than the time
that would be spent doing the multiplication.  Since the time costs of these
operations are known to the compiler in order for it to do scheduling, it is
easy for the compiler to determine when this optimization is worth using.}.
\cite{magenheimer:precision}

\section{Other optimizations}

\subsection{Low-level parallelism}

The current trend is towards duplicating hardware at the lowest level to
provide parallelism\footnote{This can been seen in the i860; floating point
additions and multiplications can proceed at the same time, and the RISC
core be moving data in and out of the floating point registers and providing
flow control at the same time the floating point units are active. \cite{byte:i860}}

Conceptually, it is easy to take advantage to low-level parallelism in the
instruction stream by simply adding more functional units to the $\mu$FPU,
widening the instruction word to control them, and then scheduling as many
operations to take place at one time as possible.

However, simply adding more functional units can only be done so many times;
there is only a limited amount of parallelism directly available in the
instruction stream, and without it, much of the extra resources will go to
waste.  One process used to make more instructions potentially schedulable
at any given time is ``trace scheduling''.  This technique originated in the
Bulldog compiler for the original VLIW machine, the ELI-512.
\cite{ellis:bulldog,colwell:vliw}  In trace scheduling, code can be
scheduled through many basic blocks at one time, following a single
potential ``trace'' of program execution.  In this way, instructions that
{\em might\/} be executed depending on a conditional branch further down in
the instruction stream are scheduled, allowing an increase in the potential
parallelism.  To account for the cases where the expected branch wasn't
taken, correction code is inserted after the branches to undo the effects of
any prematurely executed instructions.

\subsection{Pipeline optimizations}

In addition to having operations going on in parallel across functional
units, it is also typical to have several operations in various stages of
completion in each unit.  This pipelining allows the throughput of the
functional units to be increased, with no increase in latency.

There are several ways pipelined operations can be optimized.  On the
hardware side, support can be added to allow data to be recirculated back
into the beginning of the pipeline from the end, saving a trip through the
registers.  On the software side, the compiler can utilize several tricks to
try to fill up as many of the pipeline delay slots as possible, as
seendescribed by Gibbons. \cite{gib86}




==> handtable.tex <==
\begin{tabular}{lp{4in}}\toprule
\textsc{fs}-Letter & description of the most canonical shape\\\midrule
\fslist{a} & all fingers are flexed, with thumb touching the radial side of the hand, or extended\\ 
\fslist{b} & all fingers are extended. The thumb is hyper flexed across the palm\\ 
\fslist{c} & all the fingers are curved.\\ 
\fslist{d} & the index finger is fully extended. At least the middle finger is making contact with the thumb: the ring and pinky may be either flexed, or making contact with the thumb\\ 
\fslist{e} & the thumb is bent and hyper flexed across the palm, the index finger is bent and may be touching the thumb. The other fingers may be bent, like the index finger, or flexed completely.\\ 
\fslist{f} & contact with the index and thumb. The middle, ring, and pinky are all extended\\ 
\fslist{g} & the index finger is fully extended. All other fingers are flexed. The thumb is either extended fully, or unextended, against the middle finger.\\ 
\fslist{h} & index and middle fingers are fully extended. All others are flexed. The thumb is unextended or extended\\ 
\fslist{i} & the pinky is fully extended, all other fingers are flexed. The thumb is either hyperflexed, or unexetended, against the radial side\\ 
\fslist{j} & the pinky is fully extended, all other fingers are flexed. The thumb is either hyperflexed, or unexetended, against the radial side\\ 
\fslist{k} & the index finger is fully extended, the middle finger is extended, but bent ~90º at the joint closest to the hand\\ 
\fslist{l} & the index finger is fully extended, and the thumb is extended away from the hand. All other fingers are flexed\\ 
\fslist{m} & the index, middle, and ring fingers are closed, or flat-closed over the thumb, which is hyper flexed across the palm, possibly touching the base of the pinky and ring fingers\\ 
\fslist{n} & the index and middle fingers are closed, or flat-closed over the thumb, which is hyper flexed across the palm, possibly touching the base of the ring and middle fingers\\ 
\fslist{o} & the thumb and the index finger are touching in a curved, closed configuration. The other fingers are either in the same configuration, touching the thumb, or completely flexed.\\ 
\fslist{p} & the index finger is fully extended, the middle finger is extended, but bent ~90º at the joint closest to the hand\\ 
\fslist{q} & the index finger is fully extended. All other fingers are flexed. The thumb is either extended fully, or unextended, against the middle finger.\\ 
\fslist{r} & the index and middle fingers are extended and crossed over each other. All other fingers are flexed\\ 
\fslist{s} & all fingers are completely flexed, with thumb hyperflexed across the fist\\ 
\fslist{t} & the index finger is closed, or flat-closed over the thumb, which is hyper flexed across the palm, possibly touching the base of the middle and index fingers\footnote{There are some instances where the index finger flexes as the thumb is moving away from the base between the middle and index finger. In these cases the apogee for \fslist{t} should be marked when the index finger has started coming down, and the thumb starts moving. Frequently there looks to be a slight brush of the tip of the thumb across the proximal phalange.}\\ 
\fslist{u} & the index and middle fingers are completely extended, all other fingers are flexed, the thumb is hyperflexed across the palm\\ 
\fslist{v} & the index and middle fingers are completely extended and are spread apart, all other fingers are flexed, the thumb is hyperflexed across the palm\\ 
\fslist{w} & the index, middle, and ring fingers are completely extended and are spread apart, all other fingers are flexed, the thumb is hyperflexed across the palm\\ 
\fslist{x} & the index finger is bent similar to \fslist{e}, all other fingers are completely flexed\\ 
\fslist{y} & the pinky is fully extended, the thumb is hyper extended away from the hand. All other fingers are flexed\\ 
\fslist{z} & the index finger is fully extended, and all other fingers are flexed\\\bottomrule
\end{tabular}


==> preprocessing.tex <==
\subsection{Preprocessing}
\noindent{\bf Hand localization and segmentation}
For every signer, we trained a model for hand detection similar to that used in~\cite{kim,Liwicki-Everingham-09}. 
Using manually annotated hand regions, marked as polygonal regions of interest (ROI) in 30 frames, we fit a mixture of Gaussians $P_{hand}$ to the color of the
hand pixels in L*a*b color space. 
Using the same 30 frames, we also built a single-Gaussian color model $P_{bg}^x$ for every pixel $x$ in the image excluding pixel values in or near marked hand ROIs. 
Then, given a test frame, we label each pixel as hand or background based on an
odds ratio:  Given the color triplet $\mathbf{c}_x=[l_x,a_x,b_x]$ at pixel $x$, we assign it to hand if
\begin{equation}
  \label{eq:handodds}
  P_{hand}(\mathbf{c}_x)\pi_{hand}\,>\,
  P_{bg}^x(\mathbf{c}_x)(1-\pi_{hand}),
\end{equation}
where the prior $\pi_{hand}$ for hand size is estimated from the same 30
training frames.

Since this simple model produces rather noisy output, we next clean
it up by a sequence of filtering steps.  We suppress pixels that fall
within regions detected as faces by the Viola-Jones face detector~\cite{violajones},
since these tend to be false positives.  We also suppress pixels that
passed the log-odds test but have a low estimated value of $P_{hand}$.
These tend to correspond to movements in the scene, e.g., a signer
changing position and thus revealing previously occluded portions of the background; for such pixels the value of $P_{bg}$ may be low,
but so is $P_{hand}$. Finally, we suppress pixels outside of a
(generous) spatial region where the
signing is expected to occur. The largest surviving connected
component of the resulting binary map is treated as a mask that
defines the detected hand region. Some examples of resulting hand
regions are shown in
Figures~\ref{fig:lord} and~\ref{fig:method}. Note that while this procedure currently requires
manual annotation for a small number of frames in our offline
recognition setting, it could be fully
automated in a realistic interactive setting, by asking the subject
to place his/her hand in a few defined locations for calibration.\\

\noindent{\bf Handshape descriptors} The visual descriptor for a given hand region is obtained by
concatenation of 
histograms of oriented gradients (HOG~\cite{Dalal-Triggs-05})
descriptors, computed on a spatial pyramid of regions over 
the tight bounding box of the hand region, resized to canonical size
of 128$\times$128 pixels. Pixels outside of the
hand mask are ignored in this computation. The HOG pyramid consists of 4$\times$4,
8$\times$8, and 16$\times$16 grids, with eight orientation bins per
grid cell, resulting in 2688-dimensional descriptors. To speed
up computation, these descriptors were projected to at most 200
principal dimensions; the 
exact dimensionality in each experiment was tuned on a development set (see below).\\
  





==> sigdep.tex <==
\section{Signer-dependent experiments}
\label{sec:exp}


Our first experiments are signer-dependent recognition, that is, we train and test on the same signer, for each of four signers. 
%\noindent{\bf Experimental setup}  
For each signer, we use a 10-fold setup:  In each fold, 80\% of the data is used as a training set, 10\% as a development set for tuning parameters, and the remaining 10\% as a final test set.    
We independently tune the parameters in each fold, but to make it comparable to adaptation experiments later, we use 8 out of 10 folds to compute final test results and report the average letter error rate (LER) over that 8 folds.
For language models, we train the letter bigram language models from large online dictionaries of varying sizes that include both English words and names~\cite{csr}. 
We use HTK~\cite{htk} to implement the baseline HMM-based recognizers and SRILM~\cite{srilm} to train the language models. 
The HMM parameters (number of Gaussians per state, size of language model vocabulary, transition penalty and language model weight), as well as the dimensionality of the HOG descriptor input and HOG depth, were tuned to minimize development set letter error rates for the baseline HMM system.  All of the above parameters were kept fixed for the SCRF (in this sense the SCRF is slightly disadvantaged).  %The NN output type was tuned separately for the tandem HMM and the SCRF. 
Additional parameters tuned for the SCRF rescoring models included the N-best list sizes, type of feature functions, choice of language models, and L1 and L2 regularization parameters.  Finally, we tuned step size, maximum length of segmentations, and number of training epochs for first-pass SCRF model. 
%For DNN structure, we use three hidden layers and 3000 ReLUs~\cite{Zeiler_13a} hidden units for each hidden layer. Inputs to DNNs are concatenated 21 frames of HoG feature.

Figure~\ref{fig:LER} shows the letter recognition results. Tandem HMM \cite{kim2012} improves over a standard HMM baseline, and SCRF rescoring further improves over both HMM models and first-pass SCRF model outperform all other models. We also show the performance (frame error rate) of the shallow (single hidden layer) and deep NN classifiers in Figure~\ref{fig:frame_error}.
Note that in our experimental setup, there is some overlap of word types between training and test data.  This is a realistic setup, since in real applications some of the test words will have been previously seen and some will be new.  However, for comparison, we have also conducted the same experiments while keeping the training, development, and test vocabularies disjoint; in this modified setup, letter error rates increase by about 2-3\% overall, but the SCRFs still outperform the other models.
\begin{figure}
\includegraphics[width=1.05\linewidth]{figs/LER_dep}
\caption{Letter error rate for each signer and average letter error rate over all signers, for baseline HMM, tandem HMM, SCRF rescoring, and first-pass SCRF models.}
\label{fig:LER}
\end{figure}

\begin{figure}
\includegraphics[width=\linewidth]{figs/FRacc_dep}
\caption[Shallow (MLP) and deep neural network (DNN) classifier error rates on letter classification and linguistic (phonological) feature classification on test data for each signer]{Shallow (MLP) and deep neural network (DNN) classifier error rates on letter classification and linguistic (phonological) feature classification on test data for each signer.  The linguistic feature error rates are averaged over the six linguistic feature classification tasks. Chance error rates (based on always predicting the most common class) range from approximately 25\% to approximately 55\%.}
\label{fig:frame_error}
\end{figure}

%\input{figs/examplefig}



==> sigindep.tex <==
%\vspace{-.2in}
\section{Signer-independent experiments}
\label{sec:sigindep_exp}
In signer-independent setting, we would like to recognize fignerspelled letter sequences from a new signer, given a model trained on other signers.  For each of the four test signers, we train models on the remaining three signers. However, with such small size of training data (both numbers of signers and data set sizes) this may make the problem very hard, so we only assume small sets of data is available from a test signer with peak annotations or even only letter labels. 
%\input{dnn}
\input{table}
%We use the ASL video data set of~\cite{kim2013}, comprising four signers each fingerspelling 600 word tokens consisting of two repetitions of a 300-word list, including common English words, names, and foreign words. 
%The video was recorded at 60 frames per second.  
%Annotators marked the peak of articulation of each letter, and the annotations were converted to a ``ground-truth'' frame labeling by assuming that the letter boundaries occur mid-way between peaks.  Following \cite{kim2013}, the hand portion of each image is extracted via hand detection and segmentation using a signer-specific Gaussian color model, followed by suppression of irrelevant pixels.  The extracted hand images are resized to 128 $\times$ 128 and Histogram of Gradient (HoG) \cite{hog} features are extracted using multiple spatial grids (4 $\times$ 4, 8 $\times$ 8, and 16 $\times$ 16), followed by dimensionality reduction with principal components analysis (PCA).  
%Each grid includes eight directions and thus eight dimensions, for a total of 4 $\times$ 4 $\times$ 8 + 8 $\times$ 8 $\times$ 8 + 16 $\times$ 16 $\times$ 8 = 2688 dimensions.  We reduce dimensionalith with principal components analysis (PCA).

%We would like to recognize letter sequences from a new signer, given a model trained on other signers.  For each of the four signers, we train models on the remaining three signers. However, with such small size of training data (both numbers of signers and data set sizes) may make the problem very hard, so we only assume small sets of data is available from a test signer with only letter labels without any annotations. This is reasonable and realistic setting as a new signer is just asked to sign some given words without detailed supervision. Therefore, from the data from the test signer, we choose 10\% of data as tuning set of our statistical model. Then we use another 10\% of data from the same signer as test set. 


%\vspace{-.15in}
%\subsubsection{Frame classification}
%\vspace{-.05in}

%The initial unadapted signer-independent DNNs are trained on all but the test signer for each of the seven tasks (letters and the six phonological features). 
% The setting for DNNs are the same as before: the input is the $128$-dimensional HoG features concatenated over a $21$-frame window and three hidden layers of $3000$ ReLUs~\cite{Zeiler_13a}.  Cross-entropy training is done with a weight decay penalty of $10^{-5}$ via stochastic gradient descent (SGD) over $100$-sample minibatches for up to $30$ epochs, with dropout~\cite{Srivas_14a} at a rate of $0.5$ at each hidden layer, fixed momentum of $0.95$, and initial learning rate of $0.01$, which is halved when held-out accuracy stops improving.  These hyperparameters were tuned on held-out (signer-independent) data in initial experiments.  We pick the best-performing epoch on held-out data.  
%These DNNs outperform the shallow networks used in earlier work~\cite{kim2012,kim2013}.



\begin{figure}\centering
\centering
\vspace{-.06in}
\hspace{-.2in}\includegraphics[width=0.92\linewidth]{figs/adapt_bar3b.eps}
\vspace{-.15in}
\caption[DNN frame accuracies with and without normalization/adaptation]{DNN frame accuracies with and without normalization/adaptation.  The horizontal axis labels indicate the amount of adaptation data (0, 1, 2, 3 = none, 5\%, 10\%, 20\% of the test signer's data, corresponding to no adaptation, $\sim29$, $\sim58$, and $\sim115$ words).  GT = ground truth labels; FA = forced alignment labels; FT = fine-tuning.}
\label{fig:adapt}
\end{figure}

%Table{ref:frameacc-withspeed} compares the frame accuracies of the original signer-independent letter classification DNNs, the speed-normalized DNNs, and best adapted DNNs on each of the four signers.  For each test signer, the unadapted DNNs are trained on the remaining three signers.  The adapted DNNs use $20\%$ of the test signer's data (about 115 words) for adaptation and a disjoint $70\%$ of the test signer's data for testing.  There is significant variation in performance among signers, but the performance improvements are similar:  speed normalization provides a very modest improvement, and DNN adaptation provides a very significant one.  For the remaining experiments we report mean accuracies over signers and their standard deviations.

The initial unadapted signer-independent DNNs are trained on all but the test signer for each of the seven tasks (letters and the six phonological features). Then we consider DNN normalization and adaptation with different types and amounts of supervision.  For LIN+UP and LIN+LON, we adapt by running SGD over minibatches of $100$ samples with a fixed momentum of $0.9$ for up to $20$ epochs, with initial learning rate of $0.02$ (which is halved when accuracy stops improving on the adaptation data).  For fine-tuning, we use the same SGD procedure as for the signer-independent DNNs.  We pick the epoch with the highest accuracy on the adaptation data. %% \kl{highest acc on what data?  what is meant by no separate tuning data?}
The resulting frame accuracies are given in Fig.~\ref{fig:adapt}.  In addition, Fig.~\ref{fig:adapt} includes the result of speed normalization for the case of letter classification.  Speed normalization provides consistent but very small improvements, while adaptation gives large improvements in all settings.
% (KL)
% Using ground-truth frame labels results in larger improvement than using forced-aligned frame labels, more so for letter classification than for phonological feature classification.  
LIN+UP slightly outperforms LIN+LON, and fine-tuning outperforms both LIN+UP and LIN+LON. For letter sequence recognition, we adapt via fine-tuning using $20\%$ of the test signer's data.

In Fig.~\ref{fig:confmat}, we further analyze the DNNs via confusion matrices. One of the main effects is the large number of incorrect predictions of the non-signing classes ($<$s$>$, $<$/s$>$).  We observe the same effect with the phonological feature classifiers.  This may be due to the previously mentioned fact that non-linguistic gestures are variable and easy to confuse with signing when given a new signer's image frames.  The confusion matrices show that, as the DNNs are adapted, this is the main type of error that is corrected.



\begin{figure*}[t]
\centering
\begin{tabular}{@{}c@{\hspace{0.02\linewidth}}c@{\hspace{0.01\linewidth}}c@{\hspace{0.01\linewidth}}c@{}}
%& No Adapt. $C1$ & \caja{c}{c}{LIN+UP\\Forced-Align.} $C2$ & \caja{c}{c}{LIN+UP\\Ground Truth} $C3$ \\
No Adapt. & \caja{c}{c}{LIN+UP (Forced-Align.)} & \caja{c}{c}{LIN+UP (Ground Truth)} \\
%\rotatebox{90}{\hspace*{0em}Letter} &
\includegraphics[width=0.34\linewidth]{confusion_noadaptation_andy_task=letter.eps} & 
\includegraphics[width=0.28\linewidth]{confusion_forced_aligned_adaptation_andy_task=letter.eps} & 
\includegraphics[width=0.34\linewidth]{confusion_ground_truth_adaptation_andy_task=letter.eps} \\
\end{tabular}
\vspace{-.1in}
\caption[Confusion matrices of DNN classifiers for one test signer (Signer 1)]{Confusion matrices of DNN classifiers for one test signer (Signer 1).  $20\%$ of the test signer's data (115 words) was used for adaptation, and a disjoint $70\%$ was used to compute confusion matrices.  
%POR refers to the ``point of reference'' phonological feature~\cite{kim2012}.  
Each matrix cell is the empirical probability of the predicted class (column) given the ground-truth class (row).  The diagonal has been zeroed out for clarity.}
\label{fig:confmat}
\end{figure*}




%\vspace{-.15in}
%\subsubsection{Connected letter recognition}
%\vspace{-.05in}

Table~\ref{t:LER} shows the connected letter recognition accuracies obtained with the tandem, rescoring SCRF, and first-pass SCRF models with DNN adaptation via fine-tuning, using different types of adaptation data. For all models, we do not retrain the models with the adapted DNNs, but tune several hyperparameters\footnote{See~\cite{kim2012,kim2013,tang2015} for details of the tuning parameters.} on 10\% of the test signer's data.  The tuned models are evaluated on an unseen 10\% of the test signer's remaining data; finally, we repeat this for eight choices of tuning and test sets, covering the 80\% of the test signer's data that we do not use for adaptation, and report the mean letter accuracy over the test sets.  
%In other words, we assume a setting where we can train, ahead of time, a number of models with different hyperparameters on the multi-signer training data, and we have the opportunity to pick one of these models using a small amount of test signer data.

%The tuning parameters for the tandem model are the HoG scale, PCA dimensionality, insertion penalty, language model scale factor, and number of Gaussians.  For the rescoring SCRF, we tune L1 and L2 regularization coefficients, the type of DNN pooling function, and the choice of reference segmentation in training.  For the first-pass SCRF, we tune the optimization step size and number of epochs.

As shown in Table~\ref{t:LER}, without adaptation both tandem and SCRF models do poorly, achieving only roughly 40\% letter accuracies, with the rescoring SCRF slightly outperforming the others.  With adaptation, however, performance jumps to up to 69.7\% letter accuracy with forced-alignment adaptation labels and up to 82.7\% accuracy with ground-truth adaptation labels.  All of the adapted models perform similarly, but interestingly, the first-pass SCRF is slightly worse than the others before adaptation and better (by 4.4\% absolute) after ground-truth adaptation.  One hypothesis is that the first-pass SCRF is more dependent on the DNN performance, while the tandem model uses the original image features and the rescoring SCRF uses the tandem model hypotheses and scores.  Once the DNNs are adapted, however, the first-pass SCRF outperforms the other models.

%\begin{figure}
%\includegraphics[width=0.5\textwidth]{figs/LER_main}
%\caption{Letter Accuracies of models with no adaptation, adaptation with ground truth (GT) frame labels, and adaptation with forced alignments (FA) frame labels.}
%\label{f:LER}
%\end{figure}
 







==> tandem.tex <==
\subsection{A Tandem Model}
We base our approach to fingerspelling recognition on the popular tandem approach to speech recognition~\cite{ellis}.  In tandem-based speech recognition, multilayer perceptrons (MLPs) are trained to classify phones, and their outputs (phone posteriors) are post-processed and used as observations in a standard HMM-based recognizer with Gaussian mixture observation distributions.  The post-processing may include taking the logs of the posteriors (or simply taking the linear outputs of the MLPs rather than posteriors), applying principal components analysis, and/or appending acoustic features to the MLP outputs.

In this work, we begin with a basic adaptation of the tandem approach, where instead of phone posteriors estimated from acoustic frames, we use letter posteriors estimated from image features (described in Section~\ref{sec:experiments}).  Next, we propose a tandem model using classifiers of phonological features of fingerspelling rather than of the letters themselves.  The motivation is that, since features have fewer values, it may be possible to learn them more robustly than letters from small training sets, and certain features may be more or less difficult to classify.  This is similar to the work in speech recognition of \c{C}etin et al.~\cite{cetin}, who used articulatory feature MLP classifiers rather than phone classifiers.

We use a phonological feature set developed by Brentari~\cite{bren}, who proposed seven features for ASL handshape.  Of these, we use the six that are contrastive in fingerspelling.  The features and their values are given in Table~\ref{t:features}.  
 Example frames for values of the ``SF thumb'' feature are shown in Figure~\ref{f:feature_ex}, and entire phonological feature vectors for several letters are shown in Figure~\ref{f:example}. 
We also show examples for one of those features, thumb, in Figure~\ref{f:feature_ex}. 
The observations used in our HMMs consist of functions of the MLP posteriors for all values of all MLPs, concatenated with image appearance features.  In the feature-based tandem case, there is a total of 26 posteriors per frame; in the letter-based tandem case, there are 28 (26 letters + beginning ``silence'' + ending ``silence'').

\begin{table}[t]
\begin{center}
\begin{tabular}{|l|l|}
\hline
{\bf Feature} & {\bf Definition/Values}  \\ \hline \hline
SF point of & side of the hand where \\ 
reference & SFs are located  \\ \cline{2-2} 
(POR) & {\it SIL, radial, ulnar, radial/ulnar} \\ \hline\hline
SF joints & degree of flexion or \\
& extension of SFs  \\  \cline{2-2}
& {\it SIL, flexed:base, flexed:nonbase,} \\ & {\it flexed:base \& nonbase,} \\
& {\it stacked, crossed, spread} \\ \hline\hline
SF quantity &combinations of SFs \\ \cline{2-2}
& {\it N/A, all, one,} \\ & {\it one $>$ all, all $>$ one} \\ \hline\hline
SF thumb & thumb position  \\ \cline{2-2}
& {\it N/A, unopposed, opposed} \\ \hline\hline
SF handpart & internal parts of the hand  \\ \cline{2-2}
& {\it SIL, base, palm, ulnar} \\ \hline\hline
UF & open/closed \\ \cline{2-2}
& {\it SIL, open, closed} \\ \hline
\end{tabular}
\caption{Definitions and values of phonological features based on~\cite{bren}.  The first five features refer to the active fingers ({\it selected fingers}, SF); the last is the state of the inactive or {\it unselected} fingers (UF).  In addition to Brentari's feature values, we add a SIL (``silence'') value to features that lack an N/A value.  For more details, see~\cite{bren}.}
\label{t:features}
\end{center}
\end{table}

